Eliminating Unintended Stable Fixpoints for Hybrid Reasoning Systems

A wide variety of nonmonotonic semantics can be expressed as approximators defined under AFT (Approximation Fixpoint Theory). Using traditional AFT theory, it is not possible to define approximators that rely on information computed in previous iterations of stable revision. However, this information is rich for semantics that incorporate classical negation into nonmonotonic reasoning. In this work, we introduce a methodology resembling AFT that can utilize priorly computed upper bounds to more precisely capture semantics. We demonstrate our framework's applicability to hybrid MKNF (minimal knowledge and negation as failure) knowledge bases by extending the state-of-the-art approximator.

==> document-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}($\Rightarrow $) trivial. \par ($\Leftarrow $) It's sufficient to show $o{(T, F, U, P)}_{2, 3} \preceq ^2_p o{(T', F', U', P')}_{2,3}$. We have $o{(T, F, U, P)}_{2} = \lcomp {P}$ and $o{(T', F', U', P')}_{2} = \lcomp {P'}$. Clearly since $P' \preceq _{\LL } P$, we have $\lcomp {P} \preceq _{\LL } \lcomp {P'}$. We have $o{(T, F, U, P)}_{3} = \lcomp {T}$ and $o{(T', F', U', P')}_{3} = \lcomp {T'}$. From $T \preceq _{\LL } T'$, we have $\lcomp {T'} \preceq _{\LL } \lcomp {T}$. We conclude $(\lcomp {P}, \lcomp {T}) \preceq ^2_p (\lcomp {P'}, \lcomp {T'})$.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}We show (i) that $S(o)$ is a recurrent operator and then (ii) that $S(o)$ is $\preceq ^4_p$-monotone. (i) Let $(T, F, U, P) \in \LL ^4$. The functions $o{(\cdot , (U, P))}_{2}$ and $o{((T, F), \cdot )}_{3}$ are constant, therefore \begin {align*} S(o)(T, F, U, P)_{2,3} = (\LL \setminus P, \LL \setminus T) \end {align*} \par (ii) By \cite {tarskilatticetheoretical1955} and \cite {denecker2000approximations} the $S(o)$ operator is well-defined, that is, $o$ has fixpoints that exist when $o$ is monotone. Let $(T, F, U, P), (T', F', U', P') \in L^4$ such that $(T, F, U, P) \preceq ^4_p (T', F', U', P')$. It is sufficient to show \begin {enumerate}[(a)] \item $\lfp _{\preceq ^2_{{t}}} (o{(\cdot , (U, P))}_{1, 2}) \preceq ^2_t \lfp _{\preceq ^2_{{t}}} (o{(\cdot , (U', P'))}_{1, 2})$ \item $\lfp _{\preceq ^2_{{t}}} (o{((T', F'), \cdot )}_{3,4}) \preceq ^2_t \lfp _{\preceq ^2_{{t}}} (o{((T, F), \cdot )}_{3,4})$ \end {enumerate} (a) Let $x = \lfp _{\preceq ^2_{{t}}} (o{(\cdot , (U', P'))}_{1, 2})$. By the $\preceq ^4_p$-monotonicity of $o$, we have \begin {align*} o(x, (U, P)) \preceq ^2_t o(x, (U', P')) \end {align*} Here, $x$ is a prefixpoint of $o(\cdot , (U, P))$. $\lfp _{\preceq ^2_{{t}}} (o{(\cdot , (U, P))}_{1, 2})$ corresponds to the least prefixpoint of $o$ \cite {tarskilatticetheoretical1955}, thus $\lfp _{\preceq ^2_{{t}}} (o{(\cdot , (U, P))}_{1, 2}) \preceq ^2_t x$. A nearly identical procedure can be used to show that $\lfp _{\preceq ^2_{{t}}} (o{((T', F'), \cdot )}_{3,4}) \preceq ^2_t \lfp _{\preceq ^2_{{t}}} (o{((T, F), \cdot )}_{3,4})$. We conclude that $S(o)$ is $\preceq ^4_p$ monotone and with (i) it is a recurrent approximator.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}Let $(T, F, U, P), (T', F', U', P') \in L^4$ such that $(T, F, U, P) \preceq ^4_p (T', F', U', P')$. By \Proposition {relaxed-monotonicity}, it is sufficient to show $\Phi {(T, F, U, P)}_{1, 4} \preceq _p^2 \Phi {(T', F', U', P')}_{1, 4}$. It's sufficient to split our task into showing the following \begin {align*} & (i)~ add_0(T, P) \subseteq add_0(T', P')\\ & (ii)~ add_1(T, P) \subseteq add_1(T', P') \\ & (iii)~ add_0(P', T') \subseteq add_0(P, T)\\ & (iv)~ add_1(P', T') \subseteq add_1(P, T) \\ & (v)~ extract_0(T', F', U', P') \subseteq extract_0(T, F, U, P) \\ & (vi)~ extract_1(T', F', U', P') \subseteq extract_1(T, F, U, P) \end {align*} (i and iii) Follow directly from the monotonicity of $\OO $. (ii and iv) We show (ii). Let $\bfK a \in add_1(T, P)$. There exists a rule $r \in \P $ such that $\bodyp (r) \subseteq T$ and $\bodyn (r) \intersect P = \emptyset $. From $(T, P) \preceq ^2_p (T', P')$, we have $\bodyp (r) \subseteq T'$ and $\bodyn (r) \intersect P' = \emptyset $, thus, $\bfK a \in add_1(T', P')$. The case of (iv) is similar, however, the arguments and the relation are flipped. That is, we start with $\bodyp (r) \subseteq P'$ and $\bodyn (r) \intersect T' = \emptyset $ to conclude $\bodyp (r) \subseteq P$ and $\bodyn (r) \intersect T = \emptyset $. \par (v) With $F \subseteq F'$ and because $filter$ is $\subseteq $-monotone, we have ${filter(F) \subseteq filter(F')}$. Let $B \in filter(F)$ s.t. $B \subseteq F$. With $P' \subseteq P$, if we have $\OBO {P,~ B} \not \models \bot $, then we have $\OBO {P',~ B} \not \models \bot $. With $T \subseteq T'$ and with the monotonicity of $\OO $, we have $\OBO {T',~ B} \models \neg a$ when $\OBO {T,~ B} \models \neg a$. \par (vi) Let $\bfK a \in \KAK $ and $r \in \P $ such that $\head (r) \in F$, $\bodyn (r) \subseteq F$, and $(\bodyp (r) \setminus \{ \bfK a \}) \subseteq T$. From $(T, F) \preceq ^2_t (T', F')$, we get $\head (r) \in F'$, $\bodyn (r) \subseteq F'$, and $(\bodyp (r) \setminus \{ \bfK a \}) \subseteq T'$.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}($\Rightarrow $) (i) As an MKNF model, we have $N \subseteq M$, thus $T \subseteq P$. (ii) Because $\Phi {((T, F), (\cdot , \cdot ))}_{3}$ is a constant function, we need only show ${(\lfp _{\preceq ^2_t} \Phi {((T, F), (U, \cdot ))}_{4}) = P}$. We can see that $extract{(T, F, U, \cdot )}_4$ is $\subseteq $-antitone \footnote {For more details, see the proof of \Proposition {monotone}} , thus to conclude that for all $X \subseteq \KAK $, $extract(T, F, U, X) \intersect P = \emptyset $, it is sufficient to show $extract(T, F, U, \emptyset ) \intersect P = \emptyset $. Suppose for the sake of contradiction, we have $\bfK a \in (extract(T, F, U, X) \intersect P)$. Then either (a) $\OBO {T, B} \models \neg a$ for some $B \subseteq (\KAK \setminus P)$ or (b) there exists a rule whose head evaluates to false while the body evaluates as a non-false value. Clearly (b) contradicts the assumption $(M, N)$ is an MKNF model of $\KB $. We study (a) more closely. $\OBO {P, B}$ is consistent, therefore there exists an interpretation $I \in N$ such that $I$ assigns all atoms in $B$ to be false and all atoms in $P$ to be true. With $T \subseteq P$, we have $I \models \OBO {T, B}$, thus $I \models \neg a$. However, with $I \in N$, we have $I \models a$, a contradiction. (iii) $P = P^*$, so $\OBO {P^*}$ is consistent by the initial assumption. ($\Leftarrow $) To show that $(M, N)$ is an MKNF model of $\KB $, we must show the following: \begin {enumerate}[(a)] \item $(M, N) \mknfmodels \pi (\KB )$ \item $\forall (M', N')$ s.t. $M \subseteq M'$, $N \subseteq N'$, and $(M, N) \not = (M', N')$\\ $\exists I \in M', \langle I, (M', N'), (M, N) \rangle \not \models \pi (\KB )$ \end {enumerate} (a) Let $(P^*, U^*) = \lfp _{\preceq ^2_t}{\Phi ({(\cdot , \cdot ), ((\KAK \setminus P), T))}}_{1,2}$ We have $P \subseteq P^*$, thus $\OBO {P}$ is consistent. It follows that $(M, N) \mknfmodels \pi (\OO )$. Suppose for the sake of contradiction, $(M, N) \not \mknfmodels \pi (\P )$. Then there exists a rule $r \in \P $ such that $\bodyp (r) \subseteq P$, $\body (r) \intersect T = \emptyset $ and $\head (r) \not \in P$. We have $\head (r) \in P^*$, thus $\head (r)$ was remove from $P$ using an $extract$ function, a function which only prevents the derivation of atoms that will result in an inconsistency. Because the set $P^*$ extends $P$ with the atoms not blocked by $extract$, we have that $\OBO {P^*}$ is inconsistent, a contradiction. \par (b) Assume $(M, N) \mknfmodels \pi (\KB )$. If $extract$ were to remove atoms computed, the above would not hold, thus we have $P = P^*$. It follows that \begin {align*} (T, P) = \Big ( & \lfp _{\preceq ^2_t} \Phi ((\cdot , \cdot ), (\KAK \setminus \boxed {T}), \boxed {P})_{1,2}, \\ & \lfp _{\preceq ^2_t} \Phi ((\cdot , \cdot ), (\KAK \setminus \boxed {P}), \boxed {T})_{1,2}\Big )_{1,4} \end {align*} That is if we remove the $extract$ function from the operator, the result is identical. The remainder of the proof is very similar to the $\Psi $ approximator that $\Phi $ embeds ~\cite {liuyou2021}.\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}With \Proposition {S-monotone} and \Proposition {monotone}, $S(\Phi )$ is $\preceq ^4_p$-monotone. Thus \begin {align*} S(\Phi )({S(\Phi )({(T, P)^4})}) & \preceq ^4_p S(\Phi )({(T^*, P^*)}^4) \\ (\textrm {resp. }S(\Phi )({(T^*, P^*)}^4) & \preceq ^4_p S(\Phi )({S(\Phi )({(T, P)^4})}) \end {align*} By \Theorem {main}, $S(\Phi )({(T^*, P^*)}^4) = {(T^*, P^*)}^4$. Finally, $\preceq ^4_p$ embeds the $\preceq ^2_p$ relation (See \Definition {orderings}).\end{proof}

